Metaphors in Pre-Trained Language Models: Probing and Generalization Across Datasets and Languages

Human languages are full of metaphorical expressions. Metaphors help people understand the world by connecting new concepts and domains to more familiar ones. Large pre-trained language models (PLMs) are therefore assumed to encode metaphorical knowledge useful for NLP systems. In this paper, we investigate this hypothesis for PLMs, by probing metaphoricity information in their encodings, and by measuring the cross-lingual and cross-dataset generalization of this information. We present studies in multiple metaphor detection datasets and in four languages (i.e., English, Spanish, Russian, and Farsi). Our extensive experiments suggest that contextual representations in PLMs do encode metaphorical knowledge, and mostly in their middle layers. The knowledge is transferable between languages and datasets, especially when the annotation is consistent across training and testing sets. Our findings give helpful insights for both cognitive and NLP scientists.

==> plots/cartography_lcc_en.tex <==
\begin{figure*}[h!]
\centering
    \includegraphics[width=0.99\textwidth]{./img/lcc_en_xlm-roberta-base_True.pdf}
    \caption{Data map \cite{swayamdipta-etal-2020-dataset} and density plots for LCC$_{en}$ train set, based on edge probing over XLM-R model.}
    \label{fig:cartography_lcc_en}
\end{figure*}

==> plots/mdl_cross.tex <==
\begin{figure}[h]
\centering
    
    \begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group name=my plots,
            group size=1 by 1,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
        },
        footnotesize,
        width=7.5cm,
        height=3.9cm,
        xlabel=Layers,
        xmin=-0.5, xmax=12.5,
        scaled y ticks=false,
        yticklabel style={/pgf/number format/fixed},
        legend style={font=\tiny, at={(0.55,0.03)}, anchor=south west},
        xtick={0,1,...,12},
        xticklabels={0,1,...,12},
        tickpos=left,
        ytick align=outside,
        xtick align=outside,
        xmajorgrids,
    ]
    
    \nextgroupplot[ylabel={Compression}]
    \addplot[color=blue, mark=square*, thick]
        coordinates {
        (0, 1.6002827737319643)(1, 1.6388556613768601)(2, 1.731994636732814)(3, 1.8147342525421062)(4, 1.9151061165322223)(5, 1.9819495323648226)(6, 1.9883916258824856)(7, 1.986331130282477)(8, 1.981834465947605)(9, 1.988238519971158)(10, 1.953398126191568)(11, 1.9276032602445765)(12, 1.891150620307615)
        };
    \addplot[color=orange, mark=*, thick]
        coordinates {
        (0, 1.6560695277495212)(1, 1.7110869614805833)(2, 1.7949330233496497)(3, 1.9255136726181512)(4, 2.0254056911601652)(5, 2.070202190509757)(6, 2.1046560047900083)(7, 2.1099146034337277)(8, 2.0908513543129064)(9, 2.0983869640137987)(10, 2.09607973951845)(11, 2.0809102527127767)(12, 2.0304453824042152)
        };
    \addplot[color=cyan, mark=triangle*, thick]
        coordinates {
        (0, 1.408705514242383)(1, 1.406160675368454)(2, 1.4521101290198004)(3, 1.4956243208638138)(4, 1.5525661981322907)(5, 1.5725830740515558)(6, 1.5819560441852556)(7, 1.5897052242234733)(8, 1.5942882154810656)(9, 1.576204432117344)(10, 1.5777071637434745)(11, 1.577557210622736)(12, 1.5494943886435892)
        };
    \addplot[color=black, mark=triangle*, thick]
        coordinates {
        (0, 1.5736368420454083)(1, 1.6560680224765494)(2, 1.7429413759795882)(3, 1.9136011920109532)(4, 2.0537863899416844)(5, 2.1295337304930517)(6, 2.1763193133101573)(7, 2.1601986696534645)(8, 2.160659507098781)(9, 2.1704333417499138)(10, 2.180987043496526)(11, 2.228471248941881)(12, 2.1428473154502634)
        };

    \legend{en, es, fa, ru}
    
    \end{groupplot}
    \end{tikzpicture}

    \caption{MDL probing compression across layers of XLM-RoBERTa in different languages. \mf{2 SPAN LCC}}
    \label{fig:mdl_probing_cross}
\end{figure}

==> plots/mdl_xlm_vs_mono.tex <==
\begin{figure}[ht]
\centering
    
    \begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group name=my plots,
            group size=1 by 4,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
        },
        footnotesize,
        width=7.5cm,
        height=3.9cm,
        xlabel=Layers,
        xmin=-0.5, xmax=12.5,
        scaled y ticks=false,
        yticklabel style={/pgf/number format/fixed},
        legend style={font=\tiny, at={(0.55,0.03)}, anchor=south west},
        xtick={0,1,...,12},
        xticklabels={0,1,...,12},
        tickpos=left,
        ytick align=outside,
        xtick align=outside,
        xmajorgrids,
    ]
    
    
    % EN
    \nextgroupplot[ylabel={LCC (en)}]
    \addplot[color=blue, mark=square*, thick]
        coordinates {
        (0, 1.598712424057946)(1, 1.6397082006410704)(2, 1.7401230372251753)(3, 1.8289915563916046)(4, 1.9140178170286812)(5, 1.9797603566870092)(6, 2.003233440642542)(7, 1.9847243326057937)(8, 1.9784419727138187)(9, 2.0004466605076554)(10, 1.9636511527551124)(11, 1.9499921448506605)(12, 1.9011144752624414)
        };
    \addplot[color=orange, mark=*, thick]
        coordinates {
        (0, 1.6340617800432955)(1, 1.7421160930264228)(2, 1.7867262028600346)(3, 1.8365384095128507)(4, 1.9013351172835997)(5, 1.9271571996582275)(6, 1.9378035381680612)(7, 1.9342468729698983)(8, 1.9165266170775315)(9, 1.9003092702299422)(10, 1.9107437512925445)(11, 1.8981010630671376)(12, 1.851794343024528)
        };
    \addplot[color=cyan, mark=triangle*, thick]
        coordinates {
        (0, 1.6624906296766464)(1, 1.8504535260559452)(2, 1.8912016511699004)(3, 1.941280396833516)(4, 1.9907064599975892)(5, 2.025273154156184)(6, 2.0421615819409467)(7, 2.0028280770252853)(8, 1.9916204623708516)(9, 1.9834217551558273)(10, 1.9347242351571816)(11, 1.8983733175804698)(12, 1.847877400621186)
        };
        
    % ES
    \nextgroupplot[ylabel={es}]
    \addplot[color=blue, mark=square*, thick]
        coordinates {
        (0, 1.6603966474711827)(1, 1.7224636541942187)(2, 1.8030945380228929)(3, 1.9156801049151324)(4, 2.0154787479976046)(5, 2.0817711064604567)(6, 2.110628023063167)(7, 2.0938258890340475)(8, 2.090631780467786)(9, 2.101713081742114)(10, 2.0789766306510735)(11, 2.0935814600768397)(12, 2.0330693832536726)
        };
    \addplot[color=orange, mark=*, thick]
        coordinates {
        (0, 1.6762369158773072)(1, 1.7600291863787612)(2, 1.8541241271707056)(3, 1.9492413356464846)(4, 2.0222430889936147)(5, 2.051039386580339)(6, 2.0348995502133027)(7, 2.0292183126832466)(8, 2.02773963918022)(9, 2.0127823582224758)(10, 2.030993467254384)(11, 2.0180449313450777)(12, 1.9625656410267585)
        };
    \addplot[color=cyan, mark=triangle*, thick]
        coordinates {
        (0, 1.660036192126443)(1, 1.8042174651988157)(2, 1.8772157230450761)(3, 1.9632685281502529)(4, 1.9790033576181718)(5, 2.021519370338111)(6, 2.0106229151722204)(7, 1.97203682691576)(8, 1.955337831564955)(9, 1.9369304721545348)(10, 1.9315540404346154)(11, 1.9176848699864872)(12, 1.8661850657902501)
        };
        
    % FA
    \nextgroupplot[ylabel={fa}]
    \addplot[color=blue, mark=square*, thick]
        coordinates {
        (0, 1.4119441692295351)(1, 1.4051613955494453)(2, 1.4525537102411332)(3, 1.5008664421393108)(4, 1.545202793545278)(5, 1.5634528470878097)(6, 1.5819838813886162)(7, 1.5902372942415754)(8, 1.5894482050107297)(9, 1.5815077125051062)(10, 1.5842232896967492)(11, 1.588802757676746)(12, 1.5574702712406645)
        };
    \addplot[color=orange, mark=*, thick]
        coordinates {
        (0, 1.298257168193148)(1, 1.317314669261364)(2, 1.3436321938562286)(3, 1.384486280679805)(4, 1.4209315204723811)(5, 1.433101455232744)(6, 1.4475096948404256)(7, 1.4412185264041377)(8, 1.4295389637214164)(9, 1.4308487171176005)(10, 1.429125570739704)(11, 1.414293209918533)(12, 1.3715258882320078)
        };
    \addplot[color=cyan, mark=triangle*, thick]
        coordinates {
        (0, 1.4154202181483588)(1, 1.447241457099728)(2, 1.4782761632007992)(3, 1.5067416246698027)(4, 1.5348928957699488)(5, 1.5267913579182004)(6, 1.533342863575963)(7, 1.522867226685246)(8, 1.53191337665073)(9, 1.508908577700161)(10, 1.480940512954916)(11, 1.488684704675145)(12, 1.4484496616540359)
        };
    
    % RU
    \nextgroupplot[ylabel={ru}]
    \addplot[color=blue, mark=square*, thick]
        coordinates {
        (0, 1.5603314601713263)(1, 1.639789639747472)(2, 1.7478096992082799)(3, 1.892870579894531)(4, 2.0588813722058465)(5, 2.146838751194069)(6, 2.1501769535845114)(7, 2.161672835715167)(8, 2.1274642040666922)(9, 2.2229754645603252)(10, 2.2041266131585275)(11, 2.1927077907365797)(12, 2.1826511364146155)
        };
    \addplot[color=orange, mark=*, thick]
        coordinates {
        (0, 1.4613065202050894)(1, 1.5463556397738178)(2, 1.6312008279245214)(3, 1.731889014886924)(4, 1.844597776991505)(5, 1.8955628576250323)(6, 1.9394467574585117)(7, 1.960095633003617)(8, 1.9635559368222786)(9, 1.975956358565809)(10, 1.979580561806246)(11, 1.9599111360000547)(12, 1.8783794192492171)
        };
    \addplot[color=cyan, mark=triangle*, thick]
        coordinates {
        (0, 1.6519737839227986)(1, 1.7851956950762706)(2, 1.8935805403061168)(3, 1.9956673782716507)(4, 2.054587587770261)(5, 2.0893621502615334)(6, 2.0581581075477513)(7, 1.99110172032772)(8, 1.952676854652344)(9, 1.9495348000430157)(10, 1.9367156205167226)(11, 1.885549221907135)(12, 1.7964794639670083)
        };

    \legend{XLM RoBERTa,mBERT,mono-lingual BERT}
    
    \end{groupplot}
    \end{tikzpicture}

    \caption{MDL probing compression across layers in different languages. \mf{2 SPAN LCC}}
    \label{fig:mdl_probing_xlm_vs_mono}
\end{figure}

==> plots/mlm_recall.tex <==
\definecolor{mlmcolor0}{RGB}{0, 83, 87}
\definecolor{mlmcolor2}{RGB}{85, 158, 56}
\definecolor{mlmcolor3}{RGB}{115, 176, 215}
\begin{figure*}[h]
\centering
    \begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group name=my plots,
            group size=2 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
            horizontal sep=50pt,
        },
        width=0.49\textwidth,
        height=3.9cm,
        ylabel=Recall,
    	xlabel=Ranking Limit,
        scaled y ticks=false,
        yticklabel style={/pgf/number format/fixed},
        symbolic x coords={1, 10, 100, 1000},
    	x tick label style={/pgf/number format/1000 sep=},
    	xtick={1, 10, 100, 1000},
        tickpos=left,
        ytick align=outside,
        xtick align=outside,
        xmajorgrids,
        ybar=2*\pgflinewidth,
        scaled y ticks = false,
        enlarge x limits=0.25,
        legend style={font=\small, at={(-0.15,-0.65)},anchor=north},
        legend columns=-1,
        legend image code/.code={
            \draw[#1, draw=none] (0cm,-0.2cm) rectangle (0.24cm,0.25cm);
        },
    ]
    \nextgroupplot[ylabel={en}]
    \addplot[preaction={fill, mlmcolor3}, pattern=crosshatch, pattern color=white]
    	coordinates {
    	(1, 12.7)(10, 37.5)(100, 65.9)(1000, 91.3)
    	};
    \addplot[preaction={fill, mlmcolor2}, pattern=grid, pattern color=white]
    	coordinates {
    	(1, 24.8)(10, 56.3)(100, 84.6)(1000, 97.1)
    	};
    \addplot[preaction={fill, mlmcolor0}, pattern=dots, pattern color=white]
    	coordinates {
    	(1, 28.6)(10, 62.6)(100, 86.3)(1000, 97.0)
    	};
    	
    \nextgroupplot[ylabel={fa}]
    \addplot[preaction={fill, mlmcolor3}, pattern=crosshatch, pattern color=white]
    	coordinates {
    	(1, 17.6)(10, 38.0)(100, 67.2)(1000, 92.8)
    	};
    \addplot[preaction={fill, mlmcolor2}, pattern=grid, pattern color=white]
    	coordinates {
    	(1, 21.3)(10, 51.2)(100, 79.8)(1000, 96.6)
    	};
    \addplot[preaction={fill, mlmcolor0}, pattern=dots, pattern color=white]
    	coordinates {
    	(1, 34.9)(10, 67.7)(100, 88.6)(1000, 98.5)
    	};

    \nextgroupplot[ylabel={es}]
    \addplot[preaction={fill, mlmcolor3}, pattern=crosshatch, pattern color=white]
    	coordinates {
    	(1, 15.6)(10, 40.0)(100, 69.8)(1000, 95.5)
    	};
    \addplot[preaction={fill, mlmcolor2}, pattern=grid, pattern color=white]
    	coordinates {
    	(1, 27.2)(10, 61.5)(100, 86.7)(1000, 97.7)
    	};
    \addplot[preaction={fill, mlmcolor0}, pattern=dots, pattern color=white]
    	coordinates {
    	(1, 36.1)(10, 71.7)(100, 92.4)(1000, 98.8)
    	};
    	
    \nextgroupplot[ylabel={ru}]
    \addplot[preaction={fill, mlmcolor3}, pattern=crosshatch, pattern color=white]
    	coordinates {
    	(1, 17.5)(10, 48.7)(100, 73.4)(1000, 90.9)
    	};
    \addplot[preaction={fill, mlmcolor2}, pattern=grid, pattern color=white]
    	coordinates {
    	(1, 35.1)(10, 67.7)(100, 87.4)(1000, 97.9)
    	};
    \addplot[preaction={fill, mlmcolor0}, pattern=dots, pattern color=white]
    	coordinates {
    	(1, 46.5)(10, 78.9)(100, 93.6)(1000, 99.2)
    	};
    	
    \legend{clear metaphor, likely metaphor, no metaphoricity}

    \end{groupplot}
    \end{tikzpicture}
    \caption{
    XLM-RoBERTa MLM prediction recall in LCC dataset over four languages. Recall is the proportion of the entries predicted within the ranking limit to all the entries. Scores are from the LCC dataset including no metaphoricity, likely/conventional metaphor, and clear metaphor.
    }
    \label{fig:mlm_recall}
\end{figure*}

==> tables/cartography_lcc_en_table.tex <==
\begin{table*}[h]
\centering
\tabcolsep=0.11cm
\small
\begin{tabular}{lp{7.1cm}cccc}
\toprule 
  & \textbf{Instance} & \textbf{Confidence} & \textbf{Variability} & \textbf{Gold Label} & \textbf{Our Assessment}\\
\midrule 
\multirow{8}{*}{\rotatebox{90}{ambiguous}}
& A \textbf{[dome]} of a mosque in Isfahan, Iran shown below.
& 0.717
& 0.236
& Non-metaphor
&
\\\cmidrule[0.01em](lr){2-6}
& Competitive taxation is an \textbf{[academic exercise]} at best, and propaganda at worst.
& 0.689
& 0.232
& Metaphor
&
\\\cmidrule[0.01em](lr){2-6}
& No matter how dysfunctional or repressive the Soviet Union was or wasn't compared to the United States, it did offer some effective protection to \textbf{[revolutions]} of the poor , and deterrence to U.S. bully interventions.
& 0.674
& 0.222
& Non-metaphor
& 
\\\midrule[0.03em]
\multirow{8}{*}{\rotatebox{90}{hard-to-learn}}
& But the fact is, its a \textbf{[building block]} towards more gun controls in this country in the name of globalization.
& 0.009
& 0.002
& Non-metaphor
& Metaphor
\\\cmidrule[0.01em](lr){2-6}
& A query was run to derive a sub-sample of federal poverty \textbf{[participants]} from these zip codes, resulting in n=1,916 participants.
& 0.012
& 0.001
& Metaphor
& Non-metaphor
\\\cmidrule[0.01em](lr){2-6}
& DeWine would be a strong candidate against the Democratic \textbf{[golden boy]} , Rich Cordray.
& 0.016
& 0.002
& Non-metaphor
& Metaphor
\\\midrule[0.03em]
\multirow{8}{*}{\rotatebox{90}{easy-to-learn}}
& I would certainly \textbf{[recommend]} this gun to anybody considering a tippmann a-5.
& 0.996
& 0.002
& Non-metaphor
&
\\\cmidrule[0.01em](lr){2-6}
& It's much nicer to believe that peaceful mass protests lead to the near-bloodless toppling of authoritarian regimes and the \textbf{[flowering]} of democracy .
& 0.995
& 0.002
& Metaphor
&
\\\cmidrule[0.01em](lr){2-6}
& Microfinance is a solution to the \textbf{[monster]} of poverty , and promotes leadership in service.
& 0.995
& 0.001
& Metaphor
&
 \\
\bottomrule
\end{tabular}
\caption{
Examples from LCC$_{en}$ belonging to different regions in the data map.
} 
\label{tab:lcc-cartography-examples}
\end{table*}

==> tables/cross_dataset_full.tex <==
\begin{table*}[h!t!]
\begin{center}
\begin{tabular}{ l | c c | c c | c c | c c } 
 \toprule
    & \multicolumn{2}{c|}{\textbf{LCC (en)}} & \multicolumn{2}{c|}{\textbf{TroFi}} & \multicolumn{2}{c|}{\textbf{VUA POS}} & \multicolumn{2}{c}{\textbf{VUA Verbs}} \\
     \textbf{Dataset} & F1 & Rnd. F1 & F1 & Rnd. F1 & F1 & Rnd. F1 & F1 & Rnd. F1 \\
     \midrule
     \small LCC (en)   &  00.00  & 0.00\textsubscript{0} &  88.61  & 1.93\textsubscript{6} & 88.89      & 2.02\textsubscript{6}      & \bf{89.85} & \bf{2.11\textsubscript{6}}\\
     \small TroFi      &  68.32  & 0.00\textsubscript{0} &  70.22  & 1.12\textsubscript{3} & \bf{71.62} & \bf{1.16\textsubscript{3}} & 70.67      & 1.14\textsubscript{3}  \\
     \small VUA POS    &  84.06  & 0.00\textsubscript{0} &  88.91  & 2.40\textsubscript{5} & 89.00      & 2.39\textsubscript{4}      & \bf{89.31} & \bf{2.46\textsubscript{5}} \\ 
     \small VUA Verbs  &  74.39  & 0.00\textsubscript{0} &  82.40  & 1.50\textsubscript{4} & 82.97      & \bf{1.57\textsubscript{6}} & \bf{83.25} & 1.55\textsubscript{5}  \\ 
 \bottomrule
\end{tabular}
\end{center}
\caption{
Edge probing micro-averaged f1 results for various metaphoricity datasets in BERT, RoBERTa, and ELECTRA. The edge probing results are the average of three runs. The compression result is the best across layers, and the subscript denotes the best layer.
}


\label{fig:cross-dataset-full}
\end{table*}

==> tables/error_analysis.tex <==
\begin{table*}[h!t!]
\begin{center}
\begin{tabular}{ l | c | c c | c c | c c } 
 \toprule
     & \multicolumn{1}{c|}{\textbf{Total}} & \multicolumn{2}{c|}{\textbf{BERT}} & \multicolumn{2}{c|}{\textbf{RoBERTa}} & \multicolumn{2}{c}{\textbf{ELECTRA}} \\
    \textbf{Task} & Total & Correct & Incorrect & Correct & Incorrect & Correct & Incorrect \\
     \midrule
     MNLI   
     &  7.458 
     & 7.435 & 7.579 
     & 7.346 & 8.264
     & 7.403 & 7.895 \\
     QQP
     &  3.663  
     & 3.708 & 3.195
     &   3.692    & 3.353 
     & 3.672 & 3.568 \\
     AG News
     &  16.947
     & 16.872 & 18.428 
     & 16.799 & 19.603
     & 16.872 & 18.346 \\ 
 \bottomrule
\end{tabular}
\end{center}
\caption{
    c
}


\label{fig:error}
\end{table*}

==> tables/mlm.tex <==
\begin{table*}[h!t!]
\begin{center}
\begin{tabular}{l|cccc|cccc}
\toprule
                       & \multicolumn{4}{c|}{\bf{English}} & \multicolumn{4}{c}{\bf{Spanish}}        \\
R\textbackslash{}Score & 0     & 1     & 2     & 3     & 0     & 1     & 2     & 3     \\
\midrule
10                     & 1.77  & 1.93  & 1.95  & 2.32  & 1.59  & 1.77  & 1.87  & 2.21 \\
100                    & 11.01 & 10.13 & 12.43 & 18.07 & 8.57  & 9.49  & 11.43 & 18.70 \\
1000                   & 44.62 & 37.08 & 51.63 & 113.01& 26.13 & 24.63 & 42.35 & 92.81 \\
5000                   & 96.43 & 78.53 & 97.54 & 264.92& 47.09 & 39.34 & 80.70 & 168.75\\
\toprule
                       & \multicolumn{4}{c|}{\bf{Farsi}} & \multicolumn{4}{c}{\bf{Russian}}        \\
R\textbackslash{}Score & 0     & 1     & 2     & 3     & 0     & 1     & 2     & 3     \\
\midrule
10                     & 1.57  & 1.89  & 2.09  & 2.15  & 1.20  & 1.50  & 1.55  & 1.95  \\
100                    & 9.56  & 11.91 & 14.26 & 18.96 & 5.95  & 7.66  & 9.50  & 14.46 \\
1000                   & 40.86 & 51.98 & 70.23 & 115.45& 23.28 & 24.90 & 40.71 & 88.97 \\
5000                   & 65.31 & 79.55 & 123.31& 227.19& 40.41 & 33.77 & 77.72 & 297.92\\
\bottomrule
\end{tabular}
\end{center}
\caption{
XLM-RoBERTa MLM ranking average of the source concept in LCC dataset over four languages. Scores are from the LCC dataset, 0 indicating no metaphoricity, 1 possible/weak metaphor, 2 likely/conventional metaphor, and 3 clear metaphor.
}


\label{fig:mlm}
\end{table*}

==> tables/mlm_probability.tex <==
\begin{table}[h!t!]
\begin{center}
\begin{tabular}{l|ccc}
\toprule
            & \multicolumn{3}{c}{\bf{Metaphoricity Score}}  \\
\bf{Language}    & 0 & 2 & 3  \\
\midrule
English     & .20 & .17 & .08 \\
Spanish     & .27 & .19 & .12 \\
Farsi       & .28 & .15 & .13 \\
Russian     & .37 & .27 & .15 \\
\bottomrule
\end{tabular}
\end{center}
\caption{
XLM-RoBERTa MLM average probability of the source concept in the LCC datasets over four languages. Metaphoricity scores are from the LCC dataset defined as 0: no metaphoricity, 2: likely/conventional metaphor, and 3: clear metaphor. 
The probabilities are acquired after applying softmax.
}


\label{tab:mlm_probability}
\end{table}
